An LLM-Integrated Framework for Completion, Management, and Tracing of STPA

In many safety-critical engineering domains, hazard analysis techniques are an essential part of requirement elicitation. Of the methods proposed for this task, STPA (System-Theoretic Process Analysis) represents a relatively recent development in the field. The completion, management, and traceability of this hazard analysis technique present a time-consuming challenge to the requirements and safety engineers involved. In this paper, we introduce a free, open-source software framework to build STPA models with several automated workflows powered by large language models (LLMs). In past works, LLMs have been successfully integrated into a myriad of workflows across various fields. Here, we demonstrate that LLMs can be used to complete tasks associated with STPA with a high degree of accuracy, saving the time and effort of the human engineers involved. We experimentally validate our method on real-world STPA models built by requirement engineers and researchers. The source code of our software framework is available at the following link: https://github.com/blueskysolarracing/stpa.

==> Makefile <==
DOCUMENT = main

pdf: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex  # Run twice for correct references

clean:
	rm -f $(DOCUMENT).aux $(DOCUMENT).bbl $(DOCUMENT).bcf \
	      $(DOCUMENT).blg $(DOCUMENT).log $(DOCUMENT).out \
	      $(DOCUMENT).run.xml $(DOCUMENT).toc $(DOCUMENT).lof \
	      $(DOCUMENT).lot $(DOCUMENT).nav $(DOCUMENT).snm \
	      $(DOCUMENT).vrb

cleanall: clean
	rm -f $(DOCUMENT).pdf

